What are the visual features underlying human versus machine vision?

Although Deep Convolutional Networks (DCNs) are approaching the accuracy of human observers at object recognition, it is unknown whether they leverage similar visual representations to achieve this performance. To address this, we introduce Clicktionary, a web-based game for identifying visual features used by human observers during object recognition. Importance maps derived from the game are consistent across participants and uncorrelated with image saliency measures. These results suggest that Clicktionary identifies image regions that are meaningful and diagnostic for object recognition but different than those driving eye movements. Surprisingly, Clicktionary importance maps are only weakly correlated with relevance maps derived from DCNs trained for object recognition. Our study demonstrates that the narrowing gap between the object recognition accuracy of human observers and DCNs obscures distinct visual strategies used by each to achieve this performance.

==> supplementary_v1.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{latex_figures/split_half_viz}
\end{center}
   \caption{Realization map features vary according to how efficiently a participant pair recognized images. On the left, the mean realization map from pairs with above-median efficiency in recognizing glasses (i.e. faster recognition). On the right, the mean realization map from below-median pairs. The above image is representative of the typical differences between these groups.}
\vspace{}\label{split_half_viz}
\end{figure}

Despite the strong agreement we observed between \emph{Clicktionary} participants, we found that realization maps were affected by player performance. Applying a median split to the number of bubbles it took before a student in a pair recognized an image revealed two qualitatively different realization maps (Fig.~\ref{split_half_viz}). Maps from the efficient group (i.e. number of bubbles is below median split) were sparser than those from the less efficient group. More work is needed to understand if these differences indicate increased noise from the latter group or belie different sets of visual features selected by each.
%\enlargethispage{5mm}


\begin{figure}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{latex_figures/mirc_correlations}
\end{center}
   \caption{Mean pairwise correlations between realization maps derived from humans and DCNs using images from~\cite{Ullman2016-ea}. Cells are colored according to the strength and direction of association between maps.}
\vspace{}\label{fig_mirc_corr}
\end{figure} 



\begin{figure}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{latex_figures/figure_6}
\end{center}
   \caption{A depiction of the interface at  \url{Clickme.ai} for large-scale acquisition of realization maps, and continuous measurement of its impact on DCN performance. After a certain number of clicks are accrued, the application trains the weights of MLnet, a model for predicting eye fixations, to predict realization maps in images. These maps are incorporated into VGG16 through ''cooperative training'', that will drive it towards human perception.}
\vspace{}\label{webapp}
\end{figure}

